The STEM-ECR Dataset: Grounding Scientific Entity References in STEM Scholarly Content to Authoritative Encyclopedic and Lexicographic Sources

We introduce the STEM (Science, Technology, Engineering, and Medicine) Dataset for Scientific Entity Extraction, Classification, and Resolution, version 1.0 (STEM-ECR v1.0). The STEM-ECR v1.0 dataset has been developed to provide a benchmark for the evaluation of scientific entity extraction, classification, and resolution tasks in a domain-independent fashion. It comprises abstracts in 10 STEM disciplines that were found to be the most prolific ones on a major publishing platform. We describe the creation of such a multidisciplinary corpus and highlight the obtained findings in terms of the following features: 1) a generic conceptual formalism for scientific entities in a multidisciplinary scientific context; 2) the feasibility of the domain-independent human annotation of scientific entities under such a generic formalism; 3) a performance benchmark obtainable for automatic extraction of multidisciplinary scientific entities using BERT-based neural models; 4) a delineated 3-step entity resolution procedure for human annotation of the scientific entities via encyclopedic entity linking and lexicographic word sense disambiguation; and 5) human evaluations of Babelfy returned encyclopedic links and lexicographic senses for our entities. Our findings cumulatively indicate that human annotation and automatic learning of multidisciplinary scientific concepts as well as their semantic disambiguation in a wide-ranging setting as STEM is reasonable.

==> results_and_discussion.tex <==
\begin{table}[tb]
\small
\begin{tabular}{p{2.5mm}|rrrrr}
            & \multicolumn{1}{p{10mm}}{\textsc{Process}} & \multicolumn{1}{p{10mm}}{\textsc{Method}} & \multicolumn{1}{p{12mm}}{\textsc{Material}} & \multicolumn{1}{p{7mm}}{\textsc{Data}}
            & \multicolumn{1}{p{7mm}}{\textit{Overall}} \\ \hline
$P$  & 65.5   & 45.8    & 69.2      & 60.3      & 64.3    \\
$R$  & 68.3   & 44.1    & 73.2      & 60.0     & 66.7      \\
$F1$ & 66.8   & 43.0    & 71.0      & 59.8      & 65.5       
\end{tabular}
\caption{The \textit{domain-independent} scientific entity extraction system results in terms of Precision ($P$), Recall ($R$), and F-score ($F1$) on \textsc{Process}, \textsc{Method}, \textsc{Material}, and \textsc{Data} concepts, respectively, and \textit{Overall}}
\label{table:4}
\end{table}

Table~\ref{table:4} shows an overview of the \textit{domain-independent} scientific entity extraction system results. The system achieves 65.5\% overall task $F1$. For this system, \textsc{Material} was the easiest concept to extract at 71\% $F1$ and \textsc{Method} the hardest at 43\% $F1$. Of note, \textsc{Method} is also the most underrepresented in our corpus which could in part account for its poor extraction performance.

\begin{figure}[!tb]
    \center{\includegraphics[width=\linewidth]
        {classifier_perf.pdf}}
    \caption{$F1$ per domain of the 10 \textit{domain-specific} systems (as bar plots) and of the \textit{domain-independent} system (as scatter plots) for scientific concept extraction}
    \label{fig:2}
\end{figure}

Next, we compare and contrast the 10 \textit{domain-specific}
scientific entity extraction systems for their ability to extract the entities from their own domains and in other domains. These results are shown as $F1$ scores in Figure~\ref{fig:2} where the x-axis represent the 10 test domains. Of all domains, \textit{Bio} is the most robust since the \textit{domain-dependent} classifier obtains the same performance at 0.71 $F1$ as the \textit{domain-independent} system. Further, \textit{MS} (the third-last bar in each domain) is the most generic since its classifier is top-performing in other domains as well. \textit{Mat} (the second last bar in each domain) demonstrates the lowest performance in extracting scientific entities from all domains except itself showing to be the most specialized domain. 

In general, in both settings, we have obtained stable per-fold classifiers since our systems show low $F1$ standard deviation ($\sigma$) across folds. The \textit{domain-independent} classifier has $\sigma$ of 0.0140; and $\sigma$ of the respective \textit{domain-specific} classifiers when tested on their respective domains in increasing order are: \textit{Eng} (0.035); \textit{CS} (0.046); \textit{ES} (0.056); \textit{Ast} (0.057); \textit{Agr} (0.059); \textit{Mat} (0.061); \textit{Med} (0.071); \textit{Che} (0.081); \textit{Bio} (0.09); \textit{MS} (0.113). This could in part be attributed to our use of features in the form of SciBERT embeddings for machine learning that were pretrained on scientific articles.

Finally, in Table~\ref{table:5}, we report the accuracies for entity span extraction by the \textit{domain-independent} system versus inter-annotator span agreement accuracies. We find that while the annotators performed best on \textit{Med}, automated system performance was best on \textit{CS}. On the other hand, both the manual and system performance was least on \textit{Mat}. Further, comparing just the system span extraction scores with the concept extraction scatter-plot in Figure~\ref{fig:2}, shows the same performance ranks for span extraction and concept extraction across all domains except \textit{CS} and \textit{Che}. \textit{Che} is lower ranked for spans than for types, indicating a proportion of the low type scores came from span extraction errors. For more detailed machine learning results obtained on extracting scientific entities in our corpus, we refer the reader to our related work~\cite{brack2020domain}.

\begin{table}[!htb]
\small
\centering
\begin{tabular}{|p{0.35cm}|p{1.4cm}||p{0.35cm}|p{1.4cm}||p{0.35cm}|p{1.38cm}|}
\hline
    & $Acc$    &   & $Acc$    &       & $Acc$           \\ \hline
\textit{CS}  & 0.7 (0.89)  & \textit{Bio} & 0.63 (0.89) & \textit{Che}                  & 0.56 (0.86)        \\ \hline
\textit{Eng} & 0.67 (0.87) & \textit{Ast} & 0.6 (0.77)  & \textit{Mat}                  & 0.53 (0.69)        \\ \hline
\textit{Agr} & 0.65 (0.78) & \textit{ES}  & 0.59 (0.89) & \multicolumn{2}{r|}{\multirow{2}{*}{Overall 0.62 (0.86)}} \\ \cline{1-4}
\textit{MS}  & 0.64 (0.93) & \textit{Med} & 0.59 (0.97) & \multicolumn{2}{r|}{}         \\ \hline
\end{tabular}
\caption{Per-domain and Overall scientific entity span extraction accuracies by the \textit{domain-independent} classifier and parenthesized are the inter-annotator accuracies for span annotations}
\label{table:5}
\end{table}
